Oops, I Sampled it Again: Reinterpreting Confidence Intervals in Few-Shot Learning

The predominant method for computing confidence intervals (CI) in few-shot learning (FSL) is based on sampling the tasks with replacement, i.e.\ allowing the same samples to appear in multiple tasks. This makes the CI misleading in that it takes into account the randomness of the sampler but not the data itself. To quantify the extent of this problem, we conduct a comparative analysis between CIs computed with and without replacement. These reveal a notable underestimation by the predominant method. This observation calls for a reevaluation of how we interpret confidence intervals and the resulting conclusions in FSL comparative studies. Our research demonstrates that the use of paired tests can partially address this issue. Additionally, we explore methods to further reduce the (size of the) CI by strategically sampling tasks of a specific size. We also introduce a new optimized benchmark, which can be accessed at https://github.com/RafLaf/FSL-benchmark-again

==> tables/1orm1.tex <==
\begin{tabular}{llcccc|cccc}
\toprule
vs.    & Model& \multicolumn{4}{c}{CLIP} & \multicolumn{4}{c}{DINO} \\
Model     & Method &                                LR &                               NCC &                         FTN &                         PH &                                LR &                               NCC &                          FTN &                         PH \\
\midrule
\multirow{4}{*}{CLIP} & LR &     $\times \!\times \!\times \!$ &                                   &                                  &                                   &                                  &                                  &                                  &                                \\
     & NCC &   $\checkmark\times \!\checkmark$ &     $\times \!\times \!\times \!$ &                                  &                                   &                                  &                                  &                                  &                                \\
     & FTN &   $\checkmark\times \!\checkmark$ &    $\checkmark\times \!\times \!$ &    $\times \!\times \!\times \!$ &                                   &                                  &                                  &                                  &                                \\
     & PH &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\times \!\checkmark$ &     $\times \!\times \!\times \!$ &                                  &                                  &                                  &                                \\
\midrule
\multirow{4}{*}{DINO} & LR &    $\checkmark\times \!\times \!$ &   $\checkmark\times \!\checkmark$ &  $\checkmark\times \!\checkmark$ &  $\checkmark\checkmark\checkmark$ &    $\times \!\times \!\times \!$ &                                  &                                  &                                \\
     & NCC &    $\checkmark\times \!\times \!$ &    $\checkmark\times \!\times \!$ &  $\checkmark\times \!\checkmark$ &  $\checkmark\checkmark\checkmark$ &   $\checkmark\times \!\times \!$ &    $\times \!\times \!\times \!$ &                                  &                                \\
     & FTN &    $\checkmark\times \!\times \!$ &    $\checkmark\times \!\times \!$ &   $\checkmark\times \!\times \!$ &  $\checkmark\checkmark\checkmark$ &   $\checkmark\times \!\times \!$ &    $\times \!\times \!\times \!$ &    $\times \!\times \!\times \!$ &                                \\
     & PH &    $\times \!\times \!\checkmark$ &     $\times \!\times \!\times \!$ &   $\checkmark\times \!\times \!$ &   $\checkmark\times \!\checkmark$ &  $\checkmark\times \!\checkmark$ &  $\checkmark\times \!\checkmark$ &  $\checkmark\times \!\checkmark$ &  $\times \!\times \!\times \!$ \\
\bottomrule
\end{tabular}


==> tables/boolean.tex <==
\begin{tabular}{llllll|llll}
\toprule
\multirow{2}{*}{vs.}     & Model& \multicolumn{4}{c}{CLIP} & \multicolumn{4}{c}{DINO} \\
     & Method &                                LR &                               NCC &                         finetune &                         protohead &                                LR &                               NCC &                          finetune &                         protohead \\
\midrule
\multirow{4}{*}{CLIP} & LR &     $\times \!\times \!\times \!$ &     $\times \!\times \!\times \!$ &  $\checkmark\times \!\times \!$ &    $\checkmark\times \!\times \!$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ \\
     & NCC &     $\times \!\times \!\times \!$ &     $\times \!\times \!\times \!$ &  $\checkmark\times \!\times \!$ &    $\checkmark\times \!\times \!$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ \\
     & finetune &    $\checkmark\times \!\times \!$ &    $\checkmark\times \!\times \!$ &   $\times \!\times \!\times \!$ &    $\checkmark\times \!\times \!$ &    $\checkmark\times \!\times \!$ &    $\checkmark\times \!\times \!$ &    $\checkmark\times \!\times \!$ &    $\checkmark\times \!\times \!$ \\
     & protohead &    $\checkmark\times \!\times \!$ &    $\checkmark\times \!\times \!$ &  $\checkmark\times \!\times \!$ &     $\times \!\times \!\times \!$ &   $\checkmark\times \!\checkmark$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ \\
    \midrule
\multirow{4}{*}{DINO} & LR &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\times \!\times \!$ &   $\checkmark\times \!\checkmark$ &     $\times \!\times \!\times \!$ &    $\checkmark\times \!\times \!$ &   $\checkmark\times \!\checkmark$ &   $\checkmark\times \!\checkmark$ \\
     & NCC &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\times \!\times \!$ &  $\checkmark\checkmark\checkmark$ &    $\checkmark\times \!\times \!$ &     $\times \!\times \!\times \!$ &   $\checkmark\times \!\checkmark$ &   $\checkmark\times \!\checkmark$ \\
     & finetune &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\times \!\times \!$ &  $\checkmark\checkmark\checkmark$ &   $\checkmark\times \!\checkmark$ &   $\checkmark\times \!\checkmark$ &     $\times \!\times \!\times \!$ &    $\checkmark\times \!\times \!$ \\
     & protohead &  $\checkmark\checkmark\checkmark$ &  $\checkmark\checkmark\checkmark$ &  $\checkmark\times \!\times \!$ &  $\checkmark\checkmark\checkmark$ &   $\checkmark\times \!\checkmark$ &   $\checkmark\times \!\checkmark$ &    $\checkmark\times \!\times \!$ &     $\times \!\times \!\times \!$ \\
\bottomrule
\end{tabular}


==> tables/claim_benchmarkdinov2.tex <==
\begin{tabular}{cccc}
\toprule
    &              Method &              LR &             NCC \\
Dataset & Sampling &                  &                 \\
\midrule
\midrule \multirow{3}{*}{Aircraft} & 1-shot &    0.000 ± 1.161 &  -0.552 ± 1.091 \\
           & 5-shot &   -2.286 ± 2.043 &  -1.286 ± 2.027 \\
           & 10-shot &   -4.286 ± 2.568 &  -1.224 ± 2.565 \\
\midrule \multirow{3}{*}{CUB} & 1-shot &    0.000 ± 0.000 &   0.000 ± 0.000 \\
           & 5-shot &    0.121 ± 0.247 &  -0.121 ± 0.247 \\
           & 10-shot &    0.000 ± 0.000 &   0.000 ± 0.000 \\
\midrule \multirow{3}{*}{DTD} & 1-shot &    0.976 ± 1.941 &   0.488 ± 1.191 \\
           & 5-shot &   -0.250 ± 1.979 &   0.000 ± 1.348 \\
           & 10-shot &   -3.492 ± 3.253 &  -1.270 ± 1.937 \\
\midrule \multirow{3}{*}{Fungi} & 1-shot &   -0.533 ± 0.507 &   0.235 ± 0.438 \\
           & 5-shot &   -3.098 ± 0.658 &  -2.417 ± 0.677 \\
           & 10-shot &   -2.879 ± 0.890 &  -1.753 ± 0.799 \\
\midrule \multirow{3}{*}{MSCOCO} & 1-shot &    0.450 ± 0.377 &   0.180 ± 0.306 \\
           & 5-shot &   -0.196 ± 0.187 &   0.172 ± 0.141 \\
           & 10-shot &   -1.056 ± 0.204 &  -0.202 ± 0.158 \\
\midrule \multirow{3}{*}{Omniglot} & 1-shot &   -2.111 ± 0.793 &  -0.850 ± 0.755 \\
           & 5-shot &   -1.308 ± 0.564 &  -0.973 ± 0.628 \\
           & 10-shot &   -1.788 ± 0.669 &  -0.698 ± 0.733 \\
\midrule \multirow{3}{*}{Quickdraw} & 1-shot &   -1.170 ± 0.547 &   1.760 ± 0.526 \\
           & 5-shot &   -1.028 ± 0.210 &  -0.160 ± 0.235 \\
           & 10-shot &   -1.109 ± 0.171 &  -0.266 ± 0.188 \\
\midrule \multirow{3}{*}{Traffic Signs} & 1-shot &   -0.920 ± 0.519 &   0.520 ± 0.467 \\
           & 5-shot &   -1.537 ± 0.396 &  -0.367 ± 0.395 \\
           & 10-shot &   -2.857 ± 0.453 &  -0.821 ± 0.443 \\
\midrule \multirow{3}{*}{VGG Flower} & 1-shot &    0.000 ± 0.477 &   0.000 ± 0.000 \\
           & 5-shot &    0.000 ± 0.000 &  -0.182 ± 0.378 \\
           & 10-shot &    0.260 ± 0.579 &   0.260 ± 0.579 \\
\bottomrule
\end{tabular}


==> tables/table_benchmark.tex <==
\begin{tabular}{cccc}
\toprule
    &              Method &              LR &             NCC \\
Dataset & Sampling &                  &                 \\
\midrule
\multirow{3}{*}{Aircraft} & 1-shot &    0.000 ± 1.161 &  -0.552 ± 1.091 \\
           & 5-shot &   -2.286 ± 2.043 &  -1.286 ± 2.027 \\
           & 10-shot &   -4.286 ± 2.568 &  -1.224 ± 2.565 \\
           \midrule
\multirow{3}{*}{CUB} & 1-shot &    0.000 ± 0.000 &   0.000 ± 0.000 \\
           & 5-shot &    0.121 ± 0.247 &  -0.121 ± 0.247 \\
           & 10-shot &    0.000 ± 0.000 &   0.000 ± 0.000 \\
\midrule
\multirow{3}{*}{DTD} & 1-shot &    0.976 ± 1.941 &   0.488 ± 1.191 \\
           & 5-shot &   -0.250 ± 1.979 &   0.000 ± 1.348 \\
           & 10-shot &   -3.492 ± 3.253 &  -1.270 ± 1.937 \\
           \midrule
\multirow{3}{*}{Fungi} & 1-shot &   -0.533 ± 0.507 &   0.235 ± 0.438 \\
           & 5-shot &   -3.098 ± 0.658 &  -2.417 ± 0.677 \\
           & 10-shot &   -2.879 ± 0.890 &  -1.753 ± 0.799 \\
           \midrule
\multirow{3}{*}{MSCOCO} & 1-shot &    0.450 ± 0.377 &   0.180 ± 0.306 \\
           & 5-shot &   -0.196 ± 0.187 &   0.172 ± 0.141 \\
           & 10-shot &   -1.056 ± 0.204 &  -0.202 ± 0.158 \\
           \midrule
\multirow{3}{*}{Omniglot} & 1-shot &   -2.111 ± 0.793 &  -0.850 ± 0.755 \\
           & 5-shot &   -1.308 ± 0.564 &  -0.973 ± 0.628 \\
           & 10-shot &   -1.788 ± 0.669 &  -0.698 ± 0.733 \\
           \midrule
\multirow{3}{*}{Quickdraw} & 1-shot &   -1.170 ± 0.547 &   1.760 ± 0.526 \\
           & 5-shot &   -1.028 ± 0.210 &  -0.160 ± 0.235 \\
           & 10-shot &   -1.109 ± 0.171 &  -0.266 ± 0.188 \\
           \midrule
\multirow{3}{*}{Traffic Signs} & 1-shot &   -0.920 ± 0.519 &   0.520 ± 0.467 \\
           & 5-shot &   -1.537 ± 0.396 &  -0.367 ± 0.395 \\
           & 10-shot &   -2.857 ± 0.453 &  -0.821 ± 0.443 \\
           \midrule
\multirow{3}{*}{VGG Flower} & 1-shot &    0.000 ± 0.477 &   0.000 ± 0.000 \\
           & 5-shot &    0.000 ± 0.000 &  -0.182 ± 0.378 \\
           & 10-shot &    0.260 ± 0.579 &   0.260 ± 0.579 \\
\bottomrule
\end{tabular}


==> tables/traffic_signs_intro.tex <==
\begin{tabular}{ccccc|ccc}
\toprule
vs.     & Model & \multicolumn{3}{c}{CLIP} & \multicolumn{3}{c}{DINO} \\
     & Method &                                                 LR &                                                NCC &                                           FT &                                                 LR &                                                NCC &                                           FT \\
Model & Method &                                                    &                                                    &                                                    &                                                    &                                                    &                                                    \\
\midrule
\multirow{4}{*}{CLIP} & LR &                                                    &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ &  $\textcolor{blue}{\wideequal\wideequal\wideequal}$ &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ &   $\textcolor{blue}{\wideequal\wideplus\wideplus}$ &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ \\
     & NCC &  $\textcolor{red}{\wideminus\wideequal\wideminus}$ &                                                    &  $\textcolor{blue}{\wideequal\wideequal\wideequal}$ &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ &   $\textcolor{blue}{\wideequal\wideplus\wideplus}$ &  $\textcolor{blue}{\boldsymbol{\wideminus\wideequal\wideplus}}$ \\
     & FT &  $\textcolor{red}{\wideminus\wideequal\wideminus}$ &  $\textcolor{red}{\wideminus\wideequal\wideequal}$ &                                                    &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ &   $\textcolor{blue}{\wideequal\wideplus\wideplus}$ &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ \\
     \midrule
\multirow{4}{*}{DINO} & LR &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &    $\textcolor{red}{\wideplus\wideequal\wideplus}$ &    $\textcolor{red}{\wideplus\wideequal\wideplus}$ &                                                    &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ \\
     & NCC &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &    $\textcolor{red}{\wideplus\wideequal\wideplus}$ &  $\textcolor{red}{\wideminus\wideequal\wideequal}$ &                                                    &  $\textcolor{blue}{\wideequal\wideequal\wideminus} \\
     & FT &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &  $\textcolor{red}{\wideminus\wideequal\wideequal}$ &  $\textcolor{red}{\wideequal\wideequal\wideequal}$ &                                                    \\
\bottomrule
\end{tabular}


==> tables/updated_intro_table.tex <==
%\begin{NiceTabularX}{w{c}{15mm}|cc|cc}
%\toprule
%\Block[draw]{2-1}{\diagbox{Spalte}{Zeile}}  & \multicolumn{2}{c}{CLIP} & \multicolumn{2}{c}{DINO} \\
% &  & NCC & FT & NCC & FT \\
%\midrule
%\multirow{2}{*}{CLIP} & NCC &                                                    &    \textcolor{blue}%{$\wideequal\wideequal\wideequal$} &      \textcolor{blue}{$\wideequal\wideplus\wideplus$} &   %\textcolor{blue}{\boldsymbol{$\wideminus\wideequal\wideplus$}} \\
%     & FT &  \textcolor{red}{$\wideminus\wideequal\wideequal$} &                                            %        &      \textcolor{blue}{$\wideequal\wideplus\wideplus$} &   \textcolor{blue}{$\wideequal\wideequal\wideplus$} \\
%\multirow{2}{*}{DINO} & NCC &  \textcolor{red}{$\wideplus\wideequal\wideequal$} &   \textcolor{red}%{$\wideplus\wideequal\wideplus$} &                                                    &  \textcolor{blue}{\wideequal\wideequal\wideminus$} \\
%     & FT &  \textcolor{red}{$\wideplus\wideequal\wideequal$} &  \textcolor{red}{$\wideplus\wideequal\wideequal$} &  \textcolor{red}{$\wideequal\wideequal\wideequal$} &                                                  \\
%\bottomrule
%\end{NiceTabularX}


\begin{tabular}{ccc|cc|ccc}
\toprule
     &  & \multicolumn{3}{c}{CLIP} & \multicolumn{3}{c}{DINO} \\
     &  &                                                 LR &                                                NCC &                                           FT &                                                 LR &                                                NCC &                                           FT \\
 &  &                                                    &                                                    &                                                    &                                                    &                                                    &                                                    \\
\midrule
\multirow{4}{*}{CLIP} & LR &                                                    &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ &  $\textcolor{blue}{\wideequal\wideequal\wideequal}$ &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ &   $\textcolor{blue}{\wideequal\wideplus\wideplus}$ &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ \\
     & NCC &  $\textcolor{red}{\wideminus\wideequal\wideminus}$ &                                                    &  $\textcolor{blue}{\wideequal\wideequal\wideequal}$ &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ &   $\textcolor{blue}{\wideequal\wideplus\wideplus}$ &  $\textcolor{blue}{\boldsymbol{\wideminus\wideequal\wideplus}}$ \\
     & FT &  $\textcolor{red}{\wideminus\wideequal\wideminus}$ &  $\textcolor{red}{\wideminus\wideequal\wideequal}$ &                                                    &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ &   $\textcolor{blue}{\wideequal\wideplus\wideplus}$ &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ \\
     \midrule
\multirow{4}{*}{DINO} & LR &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &    $\textcolor{red}{\wideplus\wideequal\wideplus}$ &    $\textcolor{red}{\wideplus\wideequal\wideplus}$ &                                                    &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ &  $\textcolor{blue}{\wideequal\wideequal\wideplus}$ \\
     & NCC &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &    $\textcolor{red}{\wideplus\wideequal\wideplus}$ &  $\textcolor{red}{\wideminus\wideequal\wideequal}$ &                                                    &  $\textcolor{blue}{\wideequal\wideequal\wideminus} \\
     & FT &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &   $\textcolor{red}{\wideplus\wideequal\wideequal}$ &  $\textcolor{red}{\wideminus\wideequal\wideequal}$ &  $\textcolor{red}{\wideequal\wideequal\wideequal}$ &                                                    \\
\bottomrule
\end{tabular}

